Who, What, Why and How? Towards the Monetary Incentive in Crowd Collaboration: A Case Study of Github's Sponsor Mechanism

While many forms of financial support are currently available, there are still many complaints about inadequate financing from software maintainers. In May 2019, GitHub, the world's most active social coding platform, launched the Sponsor mechanism as a step toward more deeply integrating open source development and financial support. This paper collects data on 8,028 maintainers, 13,555 sponsors, and 22,515 sponsorships and conducts a comprehensive analysis. We explore the relationship between the Sponsor mechanism and developers along four dimensions using a combination of qualitative and quantitative analysis, examining why developers participate, how the mechanism affects developer activity, who obtains more sponsorships, and what mechanism flaws developers have encountered in the process of using it. We find a long-tail effect in the act of sponsorship, with most maintainers' expectations remaining unmet, and sponsorship has only a short-term, slightly positive impact on development activity but is not sustainable. While sponsors participate in this mechanism mainly as a means of thanking the developers of OSS that they use, in practice, the social status of developers is the primary influence on the number of sponsorships. We find that both the Sponsor mechanism and open source donations have certain shortcomings and need further improvements to attract more participants.

==> tables/data-description.tex <==
\begin{table*}[htbp]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.3}
\begin{threeparttable}
\caption{Descriptive statistics of collected data}
\label{data-description}
\begin{tabular}{ c m{2cm} m{5cm} m{0.7cm} m{0.7cm} m{1.2cm} m{0.7cm} m{0.7cm} m{0.7cm}}
\toprule
 & \textbf{Name} & \textbf{Description} & \textbf{Count} & \textbf{5\%} & \textbf{Mean} & \textbf{Median} & \textbf{95\%} & \textbf{SD} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Basic}}} & \emph{user\_SA} & user who creates sponsor account & 8,021 & - & - & - & - & - \\
\cline{2-9}
 & \emph{sponsor} & user who provides donation & 13,555 & - & - & - & - & - \\
\cline{2-9}
 & \emph{maintainer} & user who receives donation & 2,909 & - & - & - & - & - \\
\cline{2-9}
 & \emph{sponsorship} & donation relationship between \emph{sponsor} and \emph{maintainer} & 22,515 & - & - & - & - & - \\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Activities}}} &
\emph{commit\_num} & number of commits created by each \emph{user\_SA} per day & XXX & - & - & - & - & -  \\
\cline{2-9}
& \emph{pr\_num} & pull requests created by each \emph{user\_SA} & XXX & - & - & - & - & - \\
\cline{2-9}
& \emph{issue\_num} & issues created by each \emph{user\_SA} & XXX & - & - & - & - & -  \\
\cline{2-9}
& \emph{issue\_comment\_num} & issue comments created by each \emph{user\_SA} & XXX & - & - & - & - & -  \\
\cline{2-9}
& \emph{pr\_comment\_num} & pull request comments created by each \emph{user\_SA} & XXX & - & - & - & - & -  \\
\cline{2-9}
& \emph{commit\_comment\_num} & commit comments created by each \emph{user\_SA} & XXX & - & - & - & - & -  \\
\cline{2-9}
& \emph{review\_action\_num} & pull request reviews conducted by each \emph{user\_SA} & XXX & - & - & - & - & -  \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item - means the value is not calculated.
\end{tablenotes}
\end{threeparttable}
\end{table*}
